Efficient Multi-stage Inference on Tabular Data

Many ML applications and products train on medium amounts of input data but get bottlenecked in real-time inference. When implementing ML systems, conventional wisdom favors segregating ML code into services queried by product code via Remote Procedure Call (RPC) APIs. This approach clarifies the overall software architecture and simplifies product code by abstracting away ML internals. However, the separation adds network latency and entails additional CPU overhead. Hence, we simplify inference algorithms and embed them into the product code to reduce network communication. For public datasets and a high-performance real-time platform that deals with tabular data, we show that over half of the inputs are often amenable to such optimization, while the remainder can be handled by the original model. By applying our optimization with AutoML to both training and inference, we reduce inference latency by 1.3x, CPU resources by 30%, and network communication between application front-end and ML back-end by about 50% for a commercial end-to-end ML platform that serves millions of real-time decisions per second.

==> automlreviews.tex <==
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{-2.5pt}}
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}

\newpage

\red{AutoML Todo list}
\begin{itemize}
\item Reviewer 1
\begin{todolist}
\item 
Potential Impact On The Field Of AutoML:
I believe the framework proposed by the authors is too problem specific and the speed-up improvements are calculated on a millisecond basis. This could potentially have an impact on an organization that spends a very large fraction of time doing predictions on a set of fixed problems which can decrease the costs of the organization as well as have positive impacts on the environment. The speed-up comes with a trade-off in performance which could make the acceptance into mission-sensitive systems less acceptable.
\item[\done]
I could not easily find what the colors stand for in Figure 7 as the description of the figure does not include the datasets (except for blue belonging to adult census in Line 215.)
\red{This has been added to the caption.}
\item[\done]
Table 1 is breaking the template.
\red{This has been fixed.}
\item[\wontfix]
Line 65 and following, I would personally not use in [reference] and I would stay consistent with the way the references are done in the rest of the paper.
\item[\done]
Line 123: Creating subsets.
If I understand correctly, for each numerical feature we have b bins, for a binary categorical feature we have 2 bins, while for categorical features we have n unique cat bins, so 
 is not the correct term, since for a categorical feature we can have either fewer or more bins, making the term neither a minimum, neither a maximum constraint.
\item[\wontfix]
Could the authors describe the number of features and bins that were discovered for the considered datasets in Table 1?
\red{We omit these for the sake of meeting the page requirements, but they are included in the hyperparameters file of our code supplement.}
\item
Is there any reason for why standard deviations were not provided for Cases 1-4 in Table 1?
\red{Maybe we just ignore this comment.}
\item[\done]
"Other datasets are a representative subset of the 20+ public datasets from [31] that we used for evaluation."
What was the criteria for filtering the datasets and only including a subset?
\red{We chose a representative subset of the datasets showing a few that worked well with our approach and a few that did not work as well.}
\item[\done]
I would like the authors to add a few more datasets to their experiment. In particular, I would request 3 interesting public datasets from the AutoML Benchmark[1], KDDCup09appetency, jasmine, Amazonemployeeaccess, and Higgs from [31] (binary classification problems that fit the experimental framework of the work).
[1] Gijsbers, P., LeDell, E., Thomas, J., Poirier, S., Bischl, B., Vanschoren, J. (2019). An open source AutoML benchmark. arXiv preprint arXiv:1907.00909.
[2] The work.
\red{I added 2 of the suggested datasets. Of the other two, one was too big for my computer and one would take too long to format. I cited the automl benchmark paper.}
\item[\done]
Line 38: decision trees still outperform on tabular datasets
I would correct decision trees to gradient boosted decision trees since by themselves decision trees are weak learners.
\item[\done]
Line 35: ML competitions with tabular data have been dominated not by deep learning models, but by gradient boosting models
I believe ML competitions quite a few times include an ensembling of DNNs and GBDTs for the top solutions.
\red{This has been included}
\item[\done]
Line 47, Deep learning tends to lose out to XGBoost on structured data and this trend is stronger when training data is limited in size.
\red{This has been omitted.}
\item[\done]
The related work section seems to be lacking, since there have been several works that argue the opposite, that deep learning outperforms tabular data and the works do not mention any trends that deep learning does not perform well when training data is limited [1][2]. From personal experience, I have not observed the trend either.
Kadra, A., Lindauer, M., Hutter, F.,  Grabocka, J. (2021). Well-tuned simple nets excel on tabular datasets. Advances in neural information processing systems, 34, 23928-23941.
Gorishniy, Y., Rubachev, I., Khrulkov, V.,  Babenko, A. (2021). Revisiting deep learning models for tabular data. Advances in Neural Information Processing Systems, 34, 18932-18943.
\red{We have expanded our related work section to account for this.}
\item
The method proposed by the authors affects a specific niche, that is an organization that needs to perform a large number of predictions continuously on an already trained model. I do not believe the proposed method affects the majority of researchers in the field of AutoML, since the time taken even without using the multi-stage inference is in the range of milliseconds. Additionally, the latency reduction comes with a performance deterioration. Moreover, preparing the method has a significant overhead on the practitioner since one needs to detect the feature importances (the authors also suggest XGBoost), then organize the data into bins, run LRwithBins and detect the correct hyperparameters based on the hyperparameter n for the number of important features and b number of bins via HPO. Lastly, the practitioner would need to detect the threshold that is also dataset specific for where the performance degrades from using LRBins and XGBoost.
\red{
In a major difference from academic ML research, industrial applications of ML spend much greater resources on inference, to support products. This can be illustrated by ChatGPT, which reportedly costs \$700M/day to run, but only tens of millions USD total to train. The cost of inference is determined by CPU/GPU resources, which are closely related to mean latency. Whether the mean CPU latency is in seconds or milliseconds, it is multiplied by the large number of queries served to obtain total resources. The economics of ML inference often determines business viability.
Additionally, user-observed latency includes network latency and that of database lookups. Many online applications require latency below the cognitive threshold of 300ms, to appear instantaneous, rather than sluggish, to the users.
}
\item
There is a larger space overhead that would be required for every dataset depending on the number of features and number of bins.
\end{todolist}

\item Reviewer 2
\begin{todolist}
\item Highlight impact
\red{
We note that real-time inference dominates resource usage in industry applications by 1-2 orders of magnitude compared to training.
In a major difference from academic ML research, industrial applications of ML spend much greater resources on inference, to support products. This can be illustrated by ChatGPT, which reportedly costs \$700M/day to run, but only tens of millions USD total to train. The cost of inference is determined by CPU/GPU resources, which are closely related to mean latency. Whether the mean CPU latency is in seconds or milliseconds, it is multiplied by the large number of queries served to obtain total resources. Additionally, user-observed latency includes network latency and that of database lookups. Many online applications require latency below the cognitive threshold of 300ms, to appear instantaneous.
}
\item
The technical aspects of the proposed approach are presented in a clear manner, but the section on the algorithm could benefit from more detail. 
\red{
We have added pseudocode and more comments in order to provide more detail.
}
\item
Some parts of the paper lack technical explanations and details, which could make it difficult for readers to fully understand the system. Moreover, while the AutoML part is mentioned, it could have been better highlighted as an important aspect of the proposed approach.
\red{
We have expanded our discussion of using AutoML.
}
\item
Additionally, the paper discusses the tradeoff between ML performance and efficiency of inference, but this aspect could have been given more attention and elaboration, especially since it is an important consideration for practical applications.
\red{limited in space}
\item
The AutoML contribution is limited since AutoML is only used as a tool in the system. Moreover, this part lacks details.
\red{we have expanded on this}
\item
Better highlight AutoML part. Try to better highlight the contribution within the global system.
\red{we have expanded on this}
\end{todolist}

\item Reviewer 3
\begin{todolist}
\item
The authors seem to relegate the AutoML task to hyperparameter tuning, when in my opinion, the work contributes to the automation of multi-stage inference systems. Clarifying the degree of contribution or the current status of that automation could be something interesting.

\item[\done]
Table 1 shows a comparison of logistic regression (LR), LRwBins, and XGBoost, but in table 2 we see the difference between xgboost and hybrid model which is confusing. Is LRwBins the hybrid model? If it is something else, shouldn't it be in table1?
\red{This has been clarified in the caption of table 1.}

\item[\done]
Table 1 leaves the margins. Perhaps you could make the columns smaller by using scientific notation in dataset "size" columns, using .01 instead of 0.01, or using some other shortcut.
\red{We appreciate the suggestion and have incorporated this in the paper.}

\item[\done]
As noted in the Clarity section, comparison between XGBoost and a hybrid model is confusing, and it is unclear if the hybrid model is the same as LRwBins or something different. Clarifying this is important to relate and improve traceability between tables 1 and 2. -More information about the experimental setup could further clarify the contributions of the work. Specifically, information about the infrastructure for the remote model and product code.
\end{todolist}

\item Reviewer 4
\begin{todolist}
\item[\done] This was the code reviewer and has been handled.
\end{todolist}

\item Reviewer 5
\begin{todolist}
\item
The paper presents a solution to an interesting problem, however the perceived importance or widespread adoption is not clearly evident. Authors do not clearly explain real-world adoption scenarios. While they mention some of the advantages(including things like hardware acceleration on edge devices), it is not clear what is scope and scale where such a problem solution will have an impact.
\red{
Both the importance and the widespread adoption of the problem we solve have been described in a recent KDD publication not shown during blind review. In particular, our ML platform is deployed for over a hundred real-time industry applications.
}

\item
The basics of the proposed approach appear to be sound. The way the algorithm is presented, is however, makes it difficult to understand the details easily. There are some design choices and ther corresponding effects not clearly explained. Partitioning the data into subregions through feature grouping is explored. Why is dimensionality reduction not considered ? Line 124: Both b and n should be kept small. But n is data dependent. b i.e quantiles are user provided. It is not clear if b same for all features. If the cardinality of categorical features is rather high, how does the approach perform ? That is not addressed. LRwBins uses hyperparameter tuning, which is a part of AutoML as the authors noted. But the overall approach does not utilize any other autoML concept significantly. In terms of novelty, a simpler model to perform inference is very similar to the idea of knowledge distillation. So the application/implementation is novel but the entire idea is not. Some of the points in the conclusion may require further consideration and explanation.

\item[\done]
Clarity is by far the most significant drawback of this paper. The worst thing is the the entire algorithm is verbosely described in Section 3, without any pseudocode. This makes it very difficult for a reader to understand the details in a linear fashion. Some of the sentences are unnecessarily long(e.g. Line 150). Figures are not very informative. In Fig 1, the authors explain a familiar concept without the insights and connections to the proposed approach in a clear manner. Similarly, Figures 3 and 4 have long winded captions that do not concisely convey the core ideas. In Figure 7, the legends are missing making it hard to interpret. The content is not organized well. Tables are few, and tables like Table 1 misses providing the main message.
\red{We added pseudocode as suggested. The long sentence was fixed. Updated Fig 1 caption to connect to LRwBins. Figure 7 legend added in caption.}

\item
The paper is interesting, but is lacking in several aspects. The narrative clarity is poor and information is not well presented which makes it difficult to understand the details. The technical aspects while sound, authors do not present edge cases or generalization study. The empirical evaluation uses only a few datasets. While some of them are sizable, the applicability of this approach in a broader scenario and different data characteristics is not clear. On the positive side, the authors provide adequate references. The analysis performed is also good, especially to compare loss of accuracy. The case of RPC causing delays in inference which is a valid problem the authors are proposing a solution for.
\end{todolist}
\end{itemize}

\clearpage
Review responses:
\begin{itemize}
\item Review 1:\\
Dear Reviewer,

Thank you for your thoughtful review and valuable feedback on our paper. We have carefully addressed your comments and made the necessary changes to improve our manuscript. Please find our detailed responses below.

Potential Impact On The Field Of AutoML:
We appreciate your insights on the potential impact of our work. We acknowledge that our method solves a specific practical challenge, but it is an important one. Industrial applications of ML often have significant resource demands for inference to support products, and our method aims to optimize the tradeoffs between performance, speed and resource usage.

Figure 7 colors:
Thank you for pointing this out. We have updated the caption to include the information about the colors and datasets in Figure 7.

Table 1 formatting:
We have fixed the formatting issue with Table 1 as you suggested.

Referencing style:
We have carefully considered your suggestion, but have decided to maintain our current referencing style for consistency throughout the paper.

Line 123: Creating subsets:
You are correct in your understanding of the binning process. We have revised the terminology in the manuscript to more accurately reflect the constraints of our binning approach.

Features and bins in Table 1:
Due to page limitations, we have not included these details in the paper. However, we have provided this information in the hyperparameters file of our code supplement, as you suggested.

Dataset selection criteria:
We chose a representative subset of the datasets showing a few that worked well with our approach and a few that did not work as well.

Additional datasets:
Thank you for suggesting additional datasets for our experiment. We have included 2 of the suggested datasets and cited the AutoML benchmark paper. Unfortunately, we were unable to include the other two datasets due to technical limitations.

Line 38, 35, 47 corrections:
We appreciate your suggestions and have made the necessary corrections in our manuscript.
We have expanded our related work section to include the papers you mentioned and to better reflect the current state of research in the field.

Method's applicability and overhead:
In a major difference from academic ML research, industrial applications of ML spend much greater resources on inference, to support products. This can be illustrated by ChatGPT, which reportedly costs \$700M/day to run, but only tens of millions USD total to train. The cost of inference is determined by CPU/GPU resources, which are closely related to mean latency. Whether the mean CPU latency is in seconds or milliseconds, it is multiplied by the large number of queries served to obtain total resources. Additionally, user-observed latency includes network latency and that of database lookups. Many online applications require latency below the cognitive threshold of 300ms, to appear instantaneous. We also clarifiy that the overhead that would be required for every dataset depending on the number of features and number of bins is small in general.

We hope that our revisions have addressed your concerns and improved the quality of our paper. Once again, we appreciate your valuable feedback and the opportunity to enhance our work.

\item Review 2:\\
Dear Reviewer,

Thank you for your valuable feedback on our paper. We appreciate your insights and have made several revisions to address your concerns. Please find our detailed responses below.

Highlight impact:
We note that real-time inference dominates resource usage in industry applications by 1-2 orders of magnitude compared to training.
In a major difference from academic ML research, industrial applications of ML spend much greater resources on inference, to support products. This can be illustrated by ChatGPT, which reportedly costs \$700M/day to run, but only tens of millions USD total to train. The cost of inference is determined by CPU/GPU resources, which are closely related to mean latency. Whether the mean CPU latency is in seconds or milliseconds, it is multiplied by the large number of queries served to obtain total resources. Additionally, user-observed latency includes network latency and that of database lookups. Many online applications require latency below the cognitive threshold of 300ms, to appear instantaneous.

Algorithm detail and clarity:
We have added pseudocode and more comments to provide a clearer and more detailed presentation of the algorithm, making it easier for readers to understand the system.

Technical explanations and AutoML integration:
We have expanded our discussion on using AutoML and its importance as an aspect of the proposed approach. This should provide a more comprehensive understanding of our system and its practical applications.

Tradeoff between ML performance and efficiency of inference:
While we would have liked to provide more attention and elaboration on this tradeoff, we are limited by the space constraints of the paper. We believe our current discussion provides a reasonable balance between exploring this tradeoff and addressing other important aspects of our work.

Once again, we appreciate your valuable feedback and the opportunity to enhance our work.

\item Review 3:\\
Thank you for the insightful comments that help improve the manuscript.
We have clarified the hybrid model confusion in the caption of table 1 and have also modified table 1 according to your comments.
Indeed, our work's contribution to AutoML is beyond hyperparameter tuning, with the main focus on configuring multistage inference to ensure proper tradeoff between efficiency and coverage.  A key empirical result is that the first stage can typically handle over 50\% of inferences, and this does not require hand tuning.
We appreciate your suggestions!

\item Review 4: Already handled.

\item Review 5:\\
Dear Reviewer,

Thank you for your valuable feedback on our paper. We appreciate your insights and have made several revisions to address your concerns. Please find our detailed responses below.

Real-world adoption and impact:
Both the importance and the widespread adoption of the problem we solve have been described in a recent KDD publication not shown during blind review. In particular, our ML platform is deployed for over a hundred real-time industry applications, with millions of inferences per second.

Algorithm clarity and design choices:
We have added pseudocode to improve the clarity of our algorithm presentation, making it easier for readers to understand the details. We have also fixed the long sentence on Line 150 and updated Figure 1 caption to better connect it to LRwBins. Additionally, we added to the Figure 7 caption clarifying the missing information.

Technical explanations and AutoML integration:
We have expanded our discussion on using AutoML and its importance as an aspect of the proposed approach. This should provide a more comprehensive understanding of our system and its practical applications.

Additional comments:
We have made efforts to improve the narrative clarity of our paper by revising sections and adding pseudocode for a better understanding of our proposed algorithm. We acknowledge that presenting edge cases and a generalization study on different data characteristics would be beneficial. However, space constraints make it difficult to include these details in the current version of our paper. 
We plan to investigate these aspects in future work to provide a more comprehensive evaluation of our approach in the arxiv version. Regarding the empirical evaluation, we have added more datasets to demonstrate the applicability of our approach in various scenarios. 

Once again, we appreciate your valuable feedback and the opportunity to enhance our work.

\item General comment:\\
Dear Reviewers,

Thank you for the time and effort you have invested in evaluating our work. We have carefully addressed the comments provided and improved our revised manuscript as a result.

Notably, most reviewers found our paper to be clear ("The authors provide a clear description of the problem they are trying to solve, and their proposed solution appears to be logically consistent with the stated problem", "The work is very well written and is very easy to read. However, it has some details that could improve clarity", "The technical aspects of the proposed approach are presented in a clear manner, but the section on the algorithm could benefit from more detail").
We further enhanced the clarity based on constructive feedback received:
\begin{itemize}
\item We added pseudocode, making it easier for readers to understand the details and follow the proposed method. 
\item We provided requested details.
\item We fixed a variety of small glitches and omissions noted by reviewers, and improved formatting as requested.
\item We added two new datasets in the empirical evaluation.
\item Admittedly, we may have understated the importance of AutoML in our original manuscript. Therefore, our revised manuscript articulates the crucial role of AutoML in the success of multistage inference --- to facilitate key tradeoffs between the two stages of inference and to configure the first stage. 
% We now provide a clearer explanation of how AutoML is integrated into our approach,
% further highlighting its significance in the overall framework.
\item We are particularly grateful to the reviewer who provided comments on our code, and we addressed those as well, making the code easier to understand and reuse.
\end{itemize}

% Finally, we elaborated on the use of AutoML in our approach, going beyond hyperparameter tuning and demonstrating its integral role in the overall system.

We also addressed several misconceptions raised by the reviewers.
\begin{itemize}
\item Optimizing inference for real-time ML systems is not a niche area but rather a mainstream concern in the industry, where efficient ML inference impacts resource consumption and affects business profitability. This is critical in a growing number of real-time ML deployments --- within Web search, ad networks, many applications in social networks, various recommendation systems, etc.
\item Optimizing mean inference latency in terms of (tens and hundreds of) milliseconds is not a limitation, but rather a typical industry context. Optimizing mean CPU latency (without increasing the parallelism) helps reduce overall CPU resources.
\item The widespread impact of our proposed solution in real-time industry applications should be clearer when we disclose our affiliation and prior publications in the published paper (but we cannot do this during blind review). Our solution is deployed in a real-time industry ML platform that performs millions inferences per second for a variety of applications with billions (with a B) users worldwide.
%We highlighted the importance and adoption of our approach in real-world scenarios, emphasizing its relevance and potential impact on a large scale. 
\end{itemize}

We trust that our revisions address the reviewers' concerns and enhance the quality of the manuscript, making it suitable for publication.

Thank you once again for your valuable feedback and the opportunity to improve our work.

The Authors

\end{itemize}


==> broader_impact_and_checklist.tex <==
\section{Broader Impact Statement}
\label{sec:broader-impact}
It is difficult to ascribe ethical impact to individual papers that focus more on general-purpose algorithms or approaches meant to optimize performance by reducing resource usage such as this paper. Since this paper focuses on an end goal of maintaining machine learning performance, while reducing the resources used to achieve this goal, we can confidently say that there are no foreseeable potential negative societal impacts that would be brought about by the publication of this paper.

While this paper uses human-derived data for testing and verification purposes, the datasets used do not contain any personally identifiable information (PII) or sensitive personally identifiable information (SPII). We use popular public datasets in order to show performance to familiar data and a few datasets internal to our company representing a company-internal service, optimize client-server data transfers within a large social network, support user authentication, and access to online resources. These datasets also conform to rules and regulations internal to our company.

We have additionally tried to make this paper as accessible as possible to all reviewers and potential audience.

% this next sentence should be included as is based on the call for papers requirement
After careful reflection, the authors have determined that this work presents no notable negative impacts to society or the environment.

% The 9 pages allocated for the main paper must include a broader impact
% statement regarding the approach, datasets and applications proposed/used in
% your paper. It should reflect on the environmental, ethical and societal
% implications of your work. The statement should require at most one page and
% must be included both at submission and camera-ready time.
%
% If authors have reflected on their work and determined that there are no
% likely negative broader impacts, they may use the following statement:
%
% After careful reflection, the authors have determined that this work presents
% no notable negative impacts to society or the environment.
%
% This section is included in the template as a default, but you can also place these
% discussions anywhere else in the main paper, e.g., in the introduction/future work.
%
% The Centre for the Governance of AI has written an excellent guide for writing
% good broader impact statements (for the NeurIPS conference) that may be a
% useful resource for AutoML-Conf authors:
%
% https://medium.com/@GovAI/a-guide-to-writing-the-neurips-impact-statement-4293b723f832

\section{Submission Checklist}

% The submission checklist is a combination of the NeurIPS '21 checklist:
%
%   https://neurips.cc/Conferences/2021/PaperInformation/PaperChecklist
%
% and the NAS checklist:
%
%   https://www.automl.org/wp-content/uploads/NAS/NAS_checklist.pdf
%
% For each question, change the default \answerTODO{} to either:
%
%     \answerYes{[justification]},
%     \answerNo{[justification]}, or
%     \answerNA{[justification]}.
%
% *You must include a brief justification to your answer,* either by
% referencing the appropriate section of your paper or providing a brief inline
% description.  For example:
%
% - Did you include the license of the code and datasets?
%   \answerYes{See Section~\ref{sec:code}.}
%
% - Did you include all the code for running experiments?
%   \answerNo{We include the code we wrote, but it depends on proprietary
%   libraries for executing on a compute cluster and as such will not be
%   runnable without modifications. We also include a runnable sequential
%   version of the code that we also report experiments in the paper with.}
%
% - Did you include the license of the datasets?
%   \answerNA{Our experiments were conducted on publicly available datasets and
%   we did not introduce new datasets.}
%
% Please note that if you answer a question with \answerNo{}, we expect that you
% compensate for it (e.g., if you cannot provide the full evaluation code, you
% should at least provide code for a minimal reproduction of the main insights
% of your paper).
%
% Please do not modify the questions and only use the provided macros for your
% answers. Note that this section does not count towards the page limit.

\begin{enumerate}
\item For all authors\dots
  %
  \begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately
    reflect the paper's contributions and scope?
    %
    \answerYes{The claims made properly reflect the scope of the paper.}
    %
  \item Did you describe the limitations of your work?
    %
    \answerYes{See Section \ref{sec:limitations}.}
    %
  \item Did you discuss any potential negative societal impacts of your work?
    %
    \answerYes{See section \ref{sec:broader-impact}.}
    %
  \item Have you read the ethics author's and review guidelines and ensured that
    your paper conforms to them? \url{https://automl.cc/ethics-accessibility/}
    %
    \answerYes{This paper conforms to the ethics guidelines.}
    %
  \end{enumerate}
  %
\item If you are including theoretical results\dots
  %
  \begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    %
    \answerNA{Theoretical results are not included.}
    %
  \item Did you include complete proofs of all theoretical results?
    %
    \answerNA{Theoretical results are not included.}
    %
  \end{enumerate}
  %
\item If you ran experiments\dots
  %
  \begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the
    main experimental results, including all requirements (e.g.,
    \texttt{requirements.txt} with explicit version), an instructive
    \texttt{README} with installation, and execution commands (either in the
    supplemental material or as a \textsc{url})?
    %
    \answerYes{The code is included with relevant data and instructions. Some results, such as the latency test in the production environment, cannot be easily replicated since it requires access to the production RPC calls.}
    %
  \item Did you include the raw results of running the given instructions on the
    given code and data?
    %
    \answerYes{The results have only been truncated for readability.}
    %
  \item Did you include scripts and commands that can be used to generate the
    figures and tables in your paper based on the raw results of the code, data,
    and instructions given?
    %
    \answerYes{The plotting functions are in the code and can be easily enabled.}
    %
  \item Did you ensure sufficient code quality such that your code can be safely
    executed and the code is properly documented?
    %
    \answerYes{The code is properly documented and the model files explain what is happening in each function and why.}
    %
  \item Did you specify all the training details (e.g., data splits,
    pre-processing, search spaces, fixed hyperparameter settings, and how they
    were chosen)?
    %
    \answerYes{This is included in the code.}
    %
  \item Did you ensure that you compared different methods (including your own)
    exactly on the same benchmarks, including the same datasets, search space,
    code for training and hyperparameters for that code?
    %
    \answerYes{All methods were evaluated on the same datasets with their optimal hyperparameters.}
    %
  \item Did you run ablation studies to assess the impact of different
    components of your approach?
    %
    \answerYes{Note the robustness of this approach in the removing the entirety of our method robustly falls back to a good model.}
    %
  \item Did you use the same evaluation protocol for the methods being compared?
    %
    \answerYes{The same protocol is always used.}
    %
  \item Did you compare performance over time?
    %
    \answerYes{Internal data that shifts over time was tested and we saw similar results.}
    %
  \item Did you perform multiple runs of your experiments and report random seeds?
    %
    \answerYes{This is found in the code.}
    %
  \item Did you report error bars (e.g., with respect to the random seed after
    running experiments multiple times)?
    %
    \answerYes{See Table \ref{tab:results}.}
    %
  \item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    %
    \answerYes{Results are compared to existing popular gradient boosting models for tabular data such as XGBoost.}
    %
  \item Did you include the total amount of compute and the type of resources
    used (e.g., type of \textsc{gpu}s, internal cluster, or cloud provider)?
    %
    \answerYes{We refer to the internal CPU resource usage throughout the paper and comment on the goal of reducing resource usage.}
    %
  \item Did you report how you tuned hyperparameters, and what time and
    resources this required (if they were not automatically tuned by your AutoML
    method, e.g. in a \textsc{nas} approach; and also hyperparameters of your
    own method)?
    %
    \answerYes{Hyperparameters are tuned in the provided code.}
    %
  \end{enumerate}
  %
\item If you are using existing assets (e.g., code, data, models) or
  curating/releasing new assets\dots
  %
  \begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    %
    \answerYes{We did cite the creators of datasets and models used.}
    %
  \item Did you mention the license of the assets?
    %
    \answerNo{We invite readers to review the source material for license information.}
    %
  \item Did you include any new assets either in the supplemental material or as
    a \textsc{url}?
    %
    \answerYes{We link to the new model source code at the end of the paper.}
    %
  \item Did you discuss whether and how consent was obtained from people whose
    data you're using/curating?
    %
    \answerYes{This is discussed in the broader impacts section.}
    %
  \item Did you discuss whether the data you are using/curating contains
    personally identifiable information or offensive content?
    %
    \answerYes{This is discussed in the broader impacts section.}
    %
  \end{enumerate}
  %
\item If you used crowdsourcing or conducted research with human subjects\dots
  %
  \begin{enumerate}
  \item Did you include the full text of instructions given to participants and
    screenshots, if applicable?
    %
    \answerNA{This is not applicable.}
    %
  \item Did you describe any potential participant risks, with links to
    Institutional Review Board (\textsc{irb}) approvals, if applicable?
    %
    \answerNA{This is not applicable.}
    %
  \item Did you include the estimated hourly wage paid to participants and the
    total amount spent on participant compensation?
    %
    \answerNA{This is not applicable.}
    %
  \end{enumerate}
\end{enumerate}


==> dac_reviews.tex <==
\section{\red{DAC Reviews that need to be addressed}}

\red{
Consolidated comments to consider:
\begin{itemize}
    \item The test data should be verified as easy and difficult before inference. However, in Table III, the latency incurred by this verification is not considered.
    \blue{
    \item This is already counted in the multi-stage inference time. I added a comment in red in Table \ref{tab:latency} for clarification.
    }
    \item In the 3rd paragraph of Section III, the authors said that test data are sorted by ROC AUC to divide them into the first and second stages. However, they did not describe how to get the RUC AUC of the test data.
    \blue{
    \item The test data is never divided as such. The test inference is described well in the Training and Inference section in section 4. The validation data separation by ROCAUC and accuracy is described well in section 3. I think no action is required.
    }
    \item In the 1st paragraph of Section III, the authors split each of the n features into b bins, but they did not describe how to extract data features. The authors should also describe how to select important features in detail.
    \blue{
    \item We state: "We first use a model-free (such as MRMR \cite{ding2005minimum}) or model-based (such as XGBoost feature importance ranking \cite{chen2016xgboost}) approach to determine the relative importance of our features." I think no action is required.
    }
    \item In the 2nd paragraph of the Introduction, the authors said that it is important to make the first-stage model simpler than the second-stage model,  please first specify what the two stages are.
    \blue{
    \item This is a good point. I added some clarification in red in the second paragraph of the intro.
    }
    \item In Fig. 1, if there is a complex data set, more linear approximations may be required to fit the nonlinear blue curve, which incurs large area overheads.
    \blue{
    \item True, but this is motivation. I think no action required.
    }
    \item In Fig. 2, the authors should specify the meaning of q and x.
    \blue{
    \item Added clarification in red in caption text.
    }
    \item In Fig. 3, the authors should describe what the task is, and why the box represented by the green column has a lot of similar data.
    \blue{
    \item I think we describe the task. I don't think it is important to discuss the green column with a lot of similar data. I think no action required.
    }
    \item In Fig, 3, a steep drop-off in performance around 50K data rows offers a good separator.  The authors should specify the data before 50K is allocated to the first stage.
    \blue{
    \item This is already stated.
    }
    \item In Fig. 4, please describe what the vertical axis represents. In addition, the distribution of scale values in XGBoost is uneven.
    \blue{
    \item I think this is described well in the figure and caption.
    }
    \item In Fig.5, the authors clarify feature selection for inference in the LRwBins model, both the opacity and integers represent the importance. The leftmost red feature has an importance of integer 171 and the color is close to transparent, while the middle red feature has an importance of integer 0 and the color is opaque. The authors did not describe how to sort the importance of features like these two. In addition, The authors should also describe how many important features are selected for the task shown in Fig. 5.
    \blue{
    \item todo
    }
    \item Fig. 6 only illustrates the meaning of the blue line, the authors should add the meaning of the red and green lines. Besides, please explain why the accuracy loss of the red line is smaller than the ROC AUC performance loss.
    \blue{
    \item todo
    }
    \item In the 1st paragraph of the Introduction, ‘make practical impact' should be corrected to ‘make practical impacts'.
    \blue{
    \item Fixed.
    }
    \item In Section III-A, ‘use the the top n important features' should be corrected to ‘use the top n important features'.
    \blue{
    \item Fixed.
    }
    \item The figures in the submission are blurred. I recommend the authors use pdf to draw figures.
    \blue{
    \item todo
    }
    \item There are many works on multi-stage/hierarchical inference, yet there is almost no discussion of related work.
    \blue{
    \item Added in the intro.
    }
    \item There is no experimental comparison to similar works.
    \blue{
    \item True, but I don't think I am going to be able to add such a comparison.
    }
    \item The work strongly motivates real-time inference but the presented technique is not real-time capable.
    \blue{
    \item I think we addressed this with recent changes.
    }
    \item Most importantly, despite many existing prior works on multi-stage/hierarchical inference [2-5], there is almost no discussion of them. Only a single related work [1] is briefly discussed in half a sentence. This is despite very similar concepts being explored in [2-5]. ([2]: use a lightweight classifier to decide whether to perform local inference with a small model or whether to offload inference via the network to a powerful model; [3 and 4]: use a lightweight model that classifies simple examples and indicates "unknown" for more complex examples, which are then classified by a powerful model; [4]: incrementally increase the size of decision forests depending on the complexity of the example). Without such discussion, the novelty of this approach is not clear. Furthermore, the experimental analysis does not compare against alternative approaches (e.g., [1,2,5]). Without such comparison, it is not clear whether the proposed technique is beneficial compared to others. Finally, the work strongly motivates real-time inference but the presented technique is not real-time capable. In the worst case, still network RPC calls are needed for inference, which is unpredictable. The authors should reduce the motivation for real-time and instead motivate for the average inference latency.
    [1] (Already cited by this work) Kraft et al. Willump: A statistically-aware end-to-end optimizer for machine learning inference. MLSys. 2020.
    [2] Samie et al. Hierarchical Classification for Constrained IoT Devices: A Case Study on Human Activity Recognition. IoT-J. 2020.
    [3] Park et al. Big/Little Deep Neural Network for Ultra Low Power Inference. CODES. 2015.
    [4] Daghero et al. Two-stage Human Activity Recognition on Microcontrollers with Decision Trees and CNNs. PRIME. 2022.
    [5] Daghero et al. Adaptive Random Forests for Energy-Efficient Inference on Microcontrollers. VLSI-SoC. 2021.
    \blue{
    \item Added related work discussion in red in the intro.
    }
    \item More ablation studies are needed.
    \blue{
    \item Maybe, but I don't think I have the time to add this.
    }
    \item The running time results should be provided.
    \blue{
    \item These are provided.
    }
\end{itemize}
}

\begin{verbatim}
REVIEWER #1

Clarity / Writing Style (1-5): 3

      Originality / Innovativeness (1-5): 3
      
    Impact of Ideas and/or Results (1-5): 2
    
            OVERALL RECOMMENDATION (1-5): 2
\end{verbatim}

Summarize shortly the contributions of the paper in your own words:
The traditional machine learning system performs data inference via Remote Procedure Call (RPC) APIs, which increases network latency and entails additional CPU costs. In this paper, the authors embed a simple model into the product code to quickly process partial inferences. When data is difficult to infer, the system calls the complex model ‘XGBoost' through the RPC API to perform more precise inference. The proposed multi-stage inference method reduces the network latency and CPU costs efficiently.

Strengths:
1. The proposed multi-stage inference method achieves large performance gain by handling half of the data within the product code, it also maintains accuracy across various tabular datasets.
2. The proposed high-performance production system can achieve a 1.3x drop in latency and a 30\% drop in CPU usage compared to the traditional method.

Weaknesses:
1. The test data should be verified as easy and difficult before inference. However, in Table III, the latency incurred by this verification is not considered.
2. In the 3rd paragraph of Section III, the authors said that test data are sorted by ROC AUC to divide them into the first and second stages. However, they did not describe how to get the RUC AUC of the test data.
3. In the 1st paragraph of Section III, the authors split each of the n features into b bins, but they did not describe how to extract data features. The authors should also describe how to select important features in detail.

Main Discussion of Paper:
1. In the 2nd paragraph of the Introduction, the authors said that it is important to make the first-stage model simpler than the second-stage model,  please first specify what the two stages are.
2. In Fig. 1, if there is a complex data set, more linear approximations may be required to fit the nonlinear blue curve, which incurs large area overheads.
3. In Fig. 2, the authors should specify the meaning of q and x.
4. In Fig. 3, the authors should describe what the task is, and why the box represented by the green column has a lot of similar data.
5. In Fig, 3, a steep drop-off in performance around 50K data rows offers a good separator.  The authors should specify the data before 50K is allocated to the first stage.
6. In Fig. 4, please describe what the vertical axis represents. In addition, the distribution of scale values in XGBoost is uneven.
7. In Fig.5, the authors clarify feature selection for inference in the LRwBins model, both the opacity and integers represent the importance. The leftmost red feature has an importance of integer 171 and the color is close to transparent, while the middle red feature has an importance of integer 0 and the color is opaque. The authors did not describe how to sort the importance of features like these two. In addition, The authors should also describe how many important features are selected for the task shown in Fig. 5.
8. Fig. 6 only illustrates the meaning of the blue line, the authors should add the meaning of the red and green lines. Besides, please explain why the accuracy loss of the red line is smaller than the ROC AUC performance loss.
9. In the 1st paragraph of the Introduction, ‘make practical impact' should be corrected to ‘make practical impacts'.
10. In Section III-A, ‘use the the top n important features' should be corrected to ‘use the top n important features'.

Most prominent Strength or Weakness:
1. The test data should be verified as easy and difficult before inference. However, in Table III, the latency incurred by this verification is not considered.

\begin{verbatim}
                            REVIEWER #2

           Clarity / Writing Style (1-5): 4
           
      Originality / Innovativeness (1-5): 4
      
    Impact of Ideas and/or Results (1-5): 4
    
            OVERALL RECOMMENDATION (1-5): 4
\end{verbatim}


Summarize shortly the contributions of the paper in your own words:
The authors argue that conventional wisdom favors segregating ML code into services queried by product code causes extra overhead and CPU costs, and therefore propose to simplify inference algorithms and embed them into the product code to reduce network communication. Such inference optimization leads to 30\% reduction in CPU resources and 1.3x reduction in mean latency for a commercial ML platform that serves millions of real-time decisions per second.

Strengths
+ ...The paper is clearly stated and well-motivated.
+ ... The proposed algorithm sounds solid.
+ ... The computation reduction is promising.
+ ... The source code is provided.

Weaknesses:
- ... LRwBins suffers from a minor performance drop compared with XGB. 
- ... The figures in the submission are blurred. I recommend the authors use pdf to draw figures.

Main Discussion of Paper:
The paper is well-motivated by the fact that the common-used method segregates ML code into services queried by product code causing extra overhead. Stemming from this motivation, the paper further proposes an efficient inference that reduces 30\% of inference time while achieving comparable performance. Overall, I believe this paper is above the acceptance bar.

Most prominent Strength or Weakness:
The paper is self-containable with good motivation, sound method and convincing results.

\begin{verbatim}
                            REVIEWER #3

           Clarity / Writing Style (1-5): 5
           
      Originality / Innovativeness (1-5): 3
      
    Impact of Ideas and/or Results (1-5): 3
    
            OVERALL RECOMMENDATION (1-5): 2
\end{verbatim}


Summarize shortly the contributions of the paper in your own words:
This work presents a two-stage inference technique to reduce the required computations for inference in the average case. They divide the feature space into areas and train a separate lightweight classifier for each area. They then decide for each area whether the lightweight classifier should be used for fast inference or whether the powerful backend classifier should be invoked to maintain high accuracy.

Strengths:
+ The evaluation was performed in a production setting.
+ The technique is well described and the source code would be released, facilitating reproducing the results.
+ The discussion of limitations and unsuccessful design explorations is helpful.

Weaknesses:
- There are many works on multi-stage/hierarchical inference, yet there is almost no discussion of related work.
- There is no experimental comparison to similar works.
- The work strongly motivates real-time inference but the presented technique is not real-time capable.

Main Discussion of Paper:
This work presents a two-stage inference technique to reduce the required computations for inference in the average case. They divide the feature space into areas and train a separate lightweight classifier (logistic regression) for each area. They then decide for each area whether the lightweight classifier should be used for fast inference or whether the powerful backend classifier should be invoked via the network to maintain high accuracy, exploiting a trade-off between average latency and average accuracy.

The technique is well described and the source code would be released, which would facilitate reproducing the results. This includes a discussion of the limitations and unsuccessful design choices, which help the reader better grasp the ideas and underlying explorations. Finally, the technique was evaluated in a production setting, which strengthens the significance of the reported improvements.

However, there are also several significant shortcomings in this work. Most importantly, despite many existing prior works on multi-stage/hierarchical inference [2-5], there is almost no discussion of them. Only a single related work [1] is briefly discussed in half a sentence. This is despite very similar concepts being explored in [2-5]. ([2]: use a lightweight classifier to decide whether to perform local inference with a small model or whether to offload inference via the network to a powerful model; [3 and 4]: use a lightweight model that classifies simple examples and indicates "unknown" for more complex examples, which are then classified by a powerful model; [4]: incrementally increase the size of decision forests depending on the complexity of the example). Without such discussion, the novelty of this approach is not clear. Furthermore, the experimental analysis does not compare against alternative approaches (e.g., [1,2,5]). Without such comparison, it is not clear!
  whether the proposed technique is beneficial compared to others. Finally, the work strongly motivates real-time inference but the presented technique is not real-time capable. In the worst case, still network RPC calls are needed for inference, which is unpredictable. The authors should reduce the motivation for real-time and instead motivate for the average inference latency.

[1] (Already cited by this work) Kraft et al. Willump: A statistically-aware end-to-end optimizer for machine learning inference. MLSys. 2020.
[2] Samie et al. Hierarchical Classification for Constrained IoT Devices: A Case Study on Human Activity Recognition. IoT-J. 2020.
[3] Park et al. Big/Little Deep Neural Network for Ultra Low Power Inference. CODES. 2015.
[4] Daghero et al. Two-stage Human Activity Recognition on Microcontrollers with Decision Trees and CNNs. PRIME. 2022.
[5] Daghero et al. Adaptive Random Forests for Energy-Efficient Inference on Microcontrollers. VLSI-SoC. 2021.

Most prominent Strength or Weakness:
Missing discussion and comparison to related work.

\begin{verbatim}
                            REVIEWER #4

           Clarity / Writing Style (1-5): 3
           
      Originality / Innovativeness (1-5): 3
      
    Impact of Ideas and/or Results (1-5): 4
    
            OVERALL RECOMMENDATION (1-5): 3
\end{verbatim}

\red{
Dan:
I think we can delete this review since we have runtime results in Table \ref{tab:latency} and I feel like we clearly state why we are getting better performance.
}

Summarize shortly the contributions of the paper in your own words:
This paper provides an efficient multi-stage inference on tabular data. It improves the efficiency of real-time inference by reducing the inference latency and CPU resource usage with a little drop in performance, such as AUC and accuracy.

Strengths:
+ The paper is well-written. It clearly states its technical contribution.
+ The experimental results are comprehensive.

Weaknesses:
- More ablation studies are needed.
- The running time results should be provided.

Main Discussion of Paper:
The authors compared XGBoost and LRwBins with the proposed multi-stage model. However, it is unclear to me which component is the major reason for improved performance. It would be good if the authors could conduct some ablation studies.
Since the paper mainly claims system-level improvement, the running time comparison should be included.

Most prominent Strength or Weakness:
Good idea with a clean presentation. But more experiments are needed.

